Early-Bird GCNs: Graph-Network Co-Optimization Towards More Efficient GCN Training and Inference via Drawing Early-Bird Lottery Tickets

Graph Convolutional Networks (GCNs) have emerged as the state-of-the-art deep learning model for representation learning on graphs. However, it remains notoriously challenging to train and inference GCNs over large graph datasets, limiting their application to large real-world graphs and hindering the exploration of deeper and more sophisticated GCN graphs. This is because as the graph size grows, the sheer number of node features and the large adjacency matrix can easily explode the required memory and data movements. To tackle the aforementioned challenges, we explore the possibility of drawing lottery tickets when sparsifying GCN graphs, i.e., subgraphs that largely shrink the adjacency matrix yet are capable of achieving accuracy comparable to or even better than their full graphs. Specifically, we for the first time discover the existence of graph early-bird (GEB) tickets that emerge at the very early stage when sparsifying GCN graphs, and propose a simple yet effective detector to automatically identify the emergence of such GEB tickets. Furthermore, we advocate graph-model co-optimization and develop a generic efficient GCN early-bird training framework dubbed GEBT that can significantly boost the efficiency of GCN training by (1) drawing joint early-bird tickets between the GCN graphs and models and (2) enabling simultaneously sparsification of both the GCN graphs and models. Experiments on various GCN models and datasets consistently validate our GEB finding and the effectiveness of our GEBT, e.g., our GEBT achieves up to 80.2% ~ 85.6% and 84.6% ~ 87.5% savings of GCN training and inference costs while offering a comparable or even better accuracy as compared to state-of-the-art methods. Our source code and supplementary appendix are available at https://github.com/RICE-EIC/Early-Bird-GCN.

==> sections/4-Experiments-Full.tex <==
\vspace{-0.3em}
\section{Experiment Results}
\vspace{-0.3em}


\subsection{Experiment Setting}
\vspace{-0.3em}

\textbf{Models and Datasets.}
% We evaluate the proposed methods over the representative full-batch training GCN algorithm \cite{kipf2017semi}
% % and mini-batch training GraphSAGE algorithm \cite{hamilton2017inductive},
% on three citation graph datasets (Cora, CiteSeer, Pumbed) \cite{sen2008collective}.
%
% update
\textcolor{blue}{
We evaluate the proposed methods over five representative GCN algorithms, i.e., GCN \cite{kipf2017semi}, GAT \cite{GAT}, GIN \cite{xu2018how}, GraphSAGE \cite{hamilton2017inductive}, and 7/14/28-layer deep ResGCNs \cite{li2020deepergcn}, on three citation graph datasets, i.e., Cora, CiteSeer, and Pubmed \cite{sen2008collective},
two inductive datasets, i.e., PPI and Reddit \cite{hamilton2017inductive},
and two large-scale graph datasets from \textit{Open Graph Benchmark (OGB)} \cite{hu2020ogb}, i.e., Ogbn-ArXiv for node classification and Ogbl-Collab for link prediction.
The statistics of these seven datasets are summarized in Tab. \ref{tab:dataset}.
We follow the default setting in \cite{kipf2017semi} and \cite{hu2020ogb} to split all the datasets. The train/test/validation split ratios for Ogbn-ArXiv and Ogbl-Collab are 54/18/28 and 92/4/4, respectively.
}

% Table generated by Excel2LaTeX from sheet 'Seetting'  
\begin{table}[!b]
  \centering
  \vspace{-1.3em}
  \caption{\textcolor{blue}{The statistics of the adopted graph datasets.}}
  \vspace{-0.5em}
  \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|}
    \hline
    \textbf{Dataset} & \textbf{Nodes} & \textbf{Edges} & \textbf{Features} & \textbf{Classes} & \textbf{Metric} \bigstrut\\
    \hline
    % IMDB-BIN & 2647 & 28624 & 136 & 2  & 1.5MB \bigstrut\\
    \hline
    Cora & 2,708 & 5,429 & 1,433 & 7   & Accuracy \\
    \hline
    Citeseer & 3,312 & 4,732 & 3,703 & 6   & Accuracy \\
    \hline
    Pubmed & 19,717 & 44,338 & 500 & 3   & Accuracy \\
    \hline
    PPI & 56,944 & 818,716 & 50 & 121   & F1 Score \\
    \hline
    Ogbn-ArXiv & 169,343 & 1,166,243 & 128 & 40 & Accuracy \bigstrut\\
    \hline
    Ogbl-Collab & 235,868 & 1,285,465 & 128 & 2 & Hits@50 \bigstrut\\
    \hline
    Reddit & 232,965 & 114,615,892 & 602 & 41 & F1 Score \bigstrut\\
    \hline
    \end{tabular}%
    }
%   \vspace{-1em}
  \label{tab:dataset}%
\end{table}%


\textbf{Training Settings.}
\textcolor{blue}{
For the three citation graph datasets and two inductive graph datasets, we follow \cite{kipf2017semi} to train all the chosen two-layer GCN models of 16 hidden units for 100 epochs using an Adam optimizer \cite{kingma2014adam} with a learning rate of 0.01.
For the graphs from OGB, we follow \cite{li2020deepergcn} to use full-batch training and test for Ogbn-ArXiv while applying mini-batch training for Ogbl-Collab by randomly partitioning the graph into 10 subgraphs and doing full-batch test. For both of these two datasets, the training/retraining takes 500 epochs using an Adam optimizer \cite{kingma2014adam} with a learning rate of 0.01. A batch normalization and a dropout with a rate of 0.5 are also used for each layer of 128 hidden dimensions.
}



% Table generated by Excel2LaTeX from sheet 'Joint EB Train'
\begin{table}[t]
  \centering
  \caption{\textcolor{blue}{GEBT vs. SOTA GCN methods on citation graphs, where $\uparrow$ and $\downarrow$ denote the improvement over original models.}
%   Best node classification performance of GEBT compared with SOTA GCN algorithms.
}
  \vspace{-0.5em}
  \resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|ccc|ccc|}
\hline
 \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{3}{c|}{\textbf{Accuracy (\%)}} & \multicolumn{3}{c|}{\textbf{Inference FLOPs (M)}} \\
\cline{2-7}  & \multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{CiteSeer}} & \multicolumn{1}{c|}{\textbf{Pumbed}} &
\multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{CiteSeer}} & \multicolumn{1}{c|}{\textbf{Pumbed}} \\
\hline
\hline
GCN & 80.9  & 69.4  & 79.0  &  77.95  & 231.6  & 203.1  \\
% \hline
GraphSAGE & 82.5  & 71.0  & 78.9  & 6239  & 19654  & 15868  \\
% \hline
GAT & 82.1  & 72.1  & 79.0  &  623.6 & 1853  & 1624 \\
% \hline
GIN & 81.6  & 70.9  & 79.1  &  77.95  & 231.6  & 203.1 \\
\hline
\textbf{GEBT (GCN)} & 81.1 ($\uparrow$0.2) & 70.5 ($\uparrow$1.1) & 78.5 ($\downarrow$0.5)  & 24.94 ($\uparrow$3.1$\times$) & 51.20 ($\uparrow$4.5$\times$) & 55.77 ($\uparrow$3.6$\times$) \\
% \hline
\textbf{GEBT (GraphSAGE)} & 82.6 ($\uparrow$0.1) & 70.7 ($\downarrow$0.3) & 78.0 ($\downarrow$0.9)  & 623.9 ($\uparrow$10$\times$)  &  1965 ($\uparrow$10$\times$)  &  4760 ($\uparrow$3.3$\times$) \\
% \hline
\textbf{GEBT (GAT)} & 82.2 ($\uparrow$0.1) & 74.1 ($\uparrow$2.0) & 79.8 ($\uparrow$0.8) &  149.5 ($\uparrow$4.2$\times$) &  381.5 ($\uparrow$4.9$\times$)  &  446.2 ($\uparrow$3.6$\times$) \\
% \hline
\textbf{GEBT (GIN)} & 82.4 ($\uparrow$0.8) & 71.4 ($\uparrow$0.5) & 79.7 ($\uparrow$0.6) &  20.24 ($\uparrow$3.8$\times$) &  90.50 ($\uparrow$2.6$\times$)  &  55.77 ($\uparrow$3.6$\times$) \\
\hline
\textbf{Overall Improv.} &  \multicolumn{3}{c|}{\textbf{$\downarrow$0.9 $\sim$ $\uparrow$2.0}} & \multicolumn{3}{c|}{\textbf{$\uparrow$2.6$\times$  $\sim$ $\uparrow$10.0$\times$}} \\
\hline
\end{tabular}%
}
\vspace{-1.5em}
\label{tab:compare_GCNs}%
\end{table}%


% We conduct two kinds of comparisons to measure the effectiveness of the proposed GEBT's improved training and inference efficiency in terms of the node classification accuracy, total training FLOPs, and inference FLOPs.
% \vspace{-0.5em}
% \begin{itemize}
% \itemsep -0.3\parsep
%     \item Comparing the proposed methods with other graph sparsifiers, including the random pruning \cite{frankle2018the} and SGCN \cite{li2020sgcn}.
%     % spectral sparsifier \cite{spielman2011spectral}.
%     \item Compare the performance of the sparsified GCNs using sparsified subgraphs with the standard SOTA GCN algorithms using unpruned graphs, including the GCN \cite{kipf2017semi}, GraphSAGE \cite{hamilton2017inductive}, GAT \cite{GAT} GIN \cite{xu2018how}, and 7/14/28-layer deep ResGCNs \cite{li2020deepergcn}.
% \end{itemize}
% \vspace{-0.5em}
%

\textbf{Baselines and Evaluation Metrics.}
\textcolor{blue}{
We evaluate the effectiveness of the proposed GEBT's improved training and inference efficiency in terms of the node classification accuracy (or F1 Score, Hits@50), inference FLOPs, and total training FLOPs, as compared to other graph sparsifiers, i.e., random pruning \cite{frankle2018the} and SGCN \cite{li2020sgcn}, and the standard SOTA GCN algorithms using unpruned graphs, including the GCN \cite{kipf2017semi}, GraphSAGE \cite{hamilton2017inductive}, GAT \cite{GAT} GIN \cite{xu2018how},
ClusterGCN \cite{chiang2019cluster}, FastGCN \cite{chen2018fastgcn}, VRGCN \cite{VRGCN}, L2-GCN \cite{you2020l2}, GTTF \cite{markowitz2021graph}, N-GCN \cite{abu2020n},
and 7/14/28-layer deep ResGCNs \cite{li2020deepergcn}.
Note that Hits@50 is only used to evaluate Ogbl-Collab since the corresponding task is to predict the future author collaboration relationships given the past collaborations, we then rank each true collaboration among a set of 100,000 randomly-sampled negative collaborations, and choose the ratio of positive edges that are ranked at K-place or above (Hits@K, K is 50 here) rather than the classification accuracy as the metric for evaluating the performance.
}


\begin{table}[t]
  \centering
%   \vspace{-1em}
%   \caption{\small Apply GEBT to SOTA GCNs and PPI dataset, where $(\uparrow)$ and $(\downarrow)$ denote the improvement over original models; ``Overall Improv.'' denotes the improvement over all SOTA baselines.}
  \caption{\textcolor{blue}{GEBT vs. SOTA efficient GCN methods on PPI.}
%   ($\uparrow$) and ($\downarrow$) denote improvement over the \textit{original} models, and ``Overall Improv.'' denotes the best improvement over all \textit{SOTA} baselines
   }
  \vspace{-0.5em}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|}
        \hline
        \multirow{2}[4]{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{PPI (56K nodes and 818K edges)}} \\
        \cline{2-4}  & \multicolumn{1}{c|}{\textbf{F1 Scores (\%)}} & \multicolumn{1}{c|}{\textbf{Inference FLOPs (G)}} & \multicolumn{1}{c|}{\textbf{Training FLOPs (T)}} \\
        \hline
        \hline
        GAT & 98.2  & 3.15  & 18.9 \\
        ResGCN & 98.5  & 47.85  & 287.1 \\
        ClusterGCN & 99.3  & 35.0  & 210.0 \\
        \hline
        GraphSAGE & 61.2  & 155.8  & 934.8 \\
        VRGCN & 97.8  & 76.75  & 460.5 \\
        GraphSAINT & 98.1  & 35.0  & 210.0 \\
        L2-GCN & 96.8  & 35.0  & 210.0 \\
        N-GCN & 65.0  & 30.42  & 182.5 \\
        \hline
        \textbf{GEBT (GAT) vs. GAT} & 98.8 ($\uparrow$0.6)  & 1.84 ($\uparrow$1.7$\times$)  & 11.2 ($\uparrow$1.7$\times$) \\
        \textbf{GEBT (ResGCN) vs. ResGCN} & 98.6 ($\uparrow$0.1)  & 24.15 ($\uparrow$2.0$\times$)  & 147.8 ($\uparrow$1.9$\times$) \\
        \textbf{GEBT (ClusterGCN) vs. ClusterGCN} & 99.2 ($\downarrow$0.1)  & 19.31 ($\uparrow$1.8$\times$)   &  118.2 ($\uparrow$1.8$\times$)  \\
        \hline
        \textbf{Overall Improv.} & \textbf{$\downarrow$0.1 $\sim$ $\uparrow$38}  & \textbf{$\uparrow$1.7$\times$ $\sim$ $\uparrow$84.1$\times$}  &  \textbf{$\uparrow$1.7$\times$ $\sim$ $\uparrow$ 83.5$\times$} \\
        \hline
    \end{tabular}%
  }
  \vspace{-1.5em}
\label{tab:ppi}%
\end{table}

% ------------------
\subsection{GEBT over SOTA Sparsifiers}
We compare the proposed GEBT with existing SOTA GCN sparsification pipelines \cite{li2020sgcn} on the three graph datasets to evaluate the effectiveness of GEBT.
Fig. \ref{fig:overall_comparison_SP} shows that GEBT consistently outperforms all competitors in terms of measured accuracies and computational costs (i.e., training and inference FLOPs) trade-offs.
Specifically, GEBT via GEB tickets achieves 24.7\% $\sim$ 32.1\% training FLOPs reduction while offering comparable accuracies (-1.4\% $\sim$ 4.9\%) across a wide range of graph pruning ratios, as compared to SGCN.
Furthermore, GEBT via joint-EB tickets even aggressively reaches 80.2\% $\sim$ 85.6\% and 84.6\% $\sim$ 87.5\% reduction in training FLOPs and inference FLOPs, respectively, over SGCN when pruning the GCN networks up to 90\% sparsity, meanwhile leading to a comparable accuracy range (-1.27\% $\sim$ 1.35\%).
This set of experiments verify (1) the efficiency benefits of the proposed GEBT framework and (2) the high-quality of the drawn GEB tickets and joint-EB tickets.

% We further visualize the retraining accuracy trajectories to demonstrate the convergence of drawn joint-EB tickets. The experiments show that ...


\begin{table}[!t]
  \centering
  \caption{\textcolor{blue}{GEBT vs. SOTA efficient GCN methods on Reddit.}
%   $\uparrow$ and $\downarrow$ denote improvement over the \textit{original} models, and ``Overall Improv.'' denotes improvement over all \textit{SOTA} baselines.
  }
  \vspace{-1em}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|}
        \hline
        \multirow{2}[4]{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{Reddit (232K nodes and 11M edges)}} \\
        \cline{2-4}  & \multicolumn{1}{c|}{\textbf{F1 Scores (\%)}} & \multicolumn{1}{c|}{\textbf{Inference FLOPs (G)}} & \multicolumn{1}{c|}{\textbf{Training FLOPs (T)}} \\
        \hline
        \hline
        GCN & 95.6  & 52.3  & 470.9 \\
        GraphSAGE & 95.4  & 2396.7  &  21570.7 \\
        \hline
        FastGCN & 93.7  & 958.7  & 8628.3 \\
        VRGCN & 96.3  & 956.6  & 8609.7 \\
        ClusterGCN & 96.6  & 226.8  & 2041.1 \\
        GraphSAINT & 96.6  & 226.8  & 2041.1 \\
        GTTF (GraphSAGE) & 95.9  & 2396.7  & 21570.7 \\
        L2-GCN & 94.0  & 226.8  & 2041.1 \\
        % PPRGo (20 \#classes) & 26.6  & -  & - \\
        \hline
        \textbf{GEBT (GCN) vs. GCN} & 95.8 ($\uparrow$0.2)  & 29.3 ($\uparrow$1.8$\times$)  & 266.9 ($\uparrow$1.7$\times$) \\
        \textbf{GEBT (GraphSAGE) vs. GraphSAGE} & 97.1 ($\uparrow$1.7)  & 1198.4 ($\uparrow$2.0$\times$) & 10929.1 ($\uparrow$2.0$\times$) \\
        \hline
        \textbf{Overall Improv.} &  \textbf{$\uparrow$0.5 $\sim$ $\uparrow$3.4} &  \textbf{$\uparrow$1.8$\times$ $\sim$ $\uparrow$81.8$\times$}   &  \textbf{$\uparrow$1.7$\times$ $\sim$ $\uparrow$80.8$\times$} \\
        \hline
    \end{tabular}%
  }
  \vspace{-1em}
\label{tab:reddit}%
\end{table}



\subsection{GEBT over SOTA GCNs}

We first compare the performance of GEBT over four SOTA GCN algorithms on three citation graphs to evaluate its benefits of sparsification. As shown in Tab. \ref{tab:compare_GCNs}, GEBT again consistently outperforms the baseline GCN algorithms in terms of efficiency-accuracy trade-offs.
Specifically, GEBT achieves 2.6$\times$ $\sim$ 10$\times$ inference FLOPs reduction,
% and 0.1\% $\sim$ 4.1\% storage savings
while offering a comparable accuracy (-0.9\% $\sim$ 2.0\%), as compared to SOTA GCN algorithms.
%
\textcolor{blue}{
We further evaluate GEBT with eight SOTA methods on two large datasets, PPI and Reddit, and show the comparisons in Tables \ref{tab:ppi} and \ref{tab:reddit}, respectively, where ($\uparrow$) and ($\downarrow$) denote improvement over the \textit{original} models, and ``Overall Improv.'' denotes the best improvement over all \textit{SOTA} baselines. 
GEBT again consistently achieves the best efficiency-accuracy trade-offs, e.g., reducing inference FLOPs (up to 84.1\%) and training FLOPs (up to 83.5\%) under comparable or even higher F1-micro scores ($\downarrow$0.1\% $\sim$ $\uparrow$38\%).
}


\begin{table}[t]
  \centering
  \caption{\textcolor{blue}{GEBT vs. SOTA ResGCNs on OGB datasets.}}
  \vspace{-1em}
  \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{\tabincell{c}{ \textbf{ResGCNs} \\ \# \textbf{layers} }}} & \multicolumn{2}{c|}{\textbf{Accuracy/Hits@50 (\%)}} & \multicolumn{2}{c|}{\textbf{Inference FLOPs (G)}} \bigstrut\\
\cline{2-5}      & \textbf{Ogbn-ArXiv} & \textbf{Ogbl-Collab} & \textbf{Ogbn-ArXiv} & \textbf{Ogbl-Collab} \bigstrut\\
    \hline
    \hline
    7 & 71.3  & 53.1  & 18.56  & 24.39 \\
    14 & 72.6 & 52.9  & 39.03  & 52.60 \\
    28 & 72.1 & 53.4  & 79.96  & 109.01 \\
    \hline
    \textbf{GEBT (7)} & 71.2 ($\downarrow$0.1)  & 52.8 ($\downarrow$0.3) & 2.69 ($\uparrow$6.9$\times$) & 5.69 ($\uparrow$4.3$\times$) \\
    \textbf{GEBT (14)} & 72.3 ($\downarrow$0.3)  & 52.7 ($\downarrow$0.2)  & 9.27 ($\uparrow$4.2$\times$) & 12.13 ($\uparrow$4.3$\times$) \\
    \textbf{GEBT (28)} & 72.7 ($\uparrow$0.6) & 53.5 ($\uparrow$0.1) & 18.92 ($\uparrow$4.2$\times$) & 14.59 ($\uparrow$7.5$\times$) \\
    \hline
    \textbf{Overall Improv.} & \multicolumn{2}{c|}{ \textbf{$\downarrow$0.3 $\sim$ $\uparrow$0.6} } & \multicolumn{2}{c|}{ \textbf{$\uparrow$4.21$\times$  $\sim$ $\uparrow$7.47$\times$} } \\
    \hline
    \end{tabular}%
  }
  \vspace{-1em}
  \label{tab:scale_up_comp}%
\end{table}%

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1.02\linewidth]{figures/mark_ogn-Page-2.pdf}
    \vspace{-1.5em}
    \caption{Testing performance's trajectories visualization for 14/28-layer ResGCNs w/ and w/o applying our GEBT versus training FLOPs when evaluated on Ogbn-ArXiv and Obgl-Collab.}
    \label{fig:trajectory}
    \vspace{-1em}
\end{figure}

% ------------------
\subsection{Scale Up to Deep GCNs and Larger Graphs}
\label{sec:sacle_up}

As shown in Tab. \ref{tab:scale_up_comp}, GEBT again consistently outperforms the baseline ResGCNs algorithms in terms of the inference efficiency-accuracy trade-offs.
Specifically, GEBT achieves 4.21$\times$ $\!\sim\！$ 7.47$\times$ inference FLOPs reduction, while offering a comparable accuracy (-0.3\% $\!\sim\!$ 0.6\%), as compared to SOTA ResGCNs of various depths (e.g., 7/14/28-layer ResGCNs).
%
Fig. \ref{fig:trajectory} (a) and (b) further visualize the testing performance's trajectories of graph early-bird tickets training (GEBT) and baseline ResGCNs training versus the training FLOPs on Ogbn-ArXiv and Ogbl-Collab datasets, respectively.
We can see that GEBT achieves a comparable accuracy with fewer training FLOPs, indicating its good generalization capability and the effectiveness of early-bird tickets and the proposed graph-network co-optimization.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Graph_EB_Distance_ablation.pdf}
    % \includegraphics[width=\linewidth]{figures/ablation_study (1).pdf}
    \includegraphics[width=\linewidth]{figures/ablation_study_crop.pdf}
    \vspace{-2em}
    \caption{The (a) recorded distance's evolution along GCN training trajetories on the Cora dataset, and (b) retraining accuracies comparisons among different identifiers, where horizontal axis denotes the network sparisty and vertical axis indicates the graph sparsity.}
    \vspace{-1em}
    \label{fig:identifier_ablation}
\end{figure}


% ------------------
\subsection{Ablation Studies of Joint-EB Detectors}
\label{sec:joint_EB_criteria}
We adopt a mixture of ``graph distance'' and ``network distance'' to identify the joint-EB tickets in all the above experiments, and are further curious about whether a detector based on one of the two distances can still lead to similar benefits.
To validate this, we first measure and compare the epoch ranges where joint-EB tickets emerge, and when applying another two criteria (1) $d_g < \eta$ and (2) $d_w < \eta$, respectively. We can see that the graph distance criterion is more suitable than the network distance criterion, because the latter undergoes a ``warming up'' process starting from 0 to 1 and then quickly drops to nearly zero, making joint-EB detection collapse to the initial training stage even if we ignore such ``warming up'' as shown in Fig. \ref{fig:identifier_ablation} (a).
Then, we compare the retraining accuracy of the drawn joint-EB tickets using all the three criteria to see their robustness to different criteria (i.e., drawing epochs). The results in Fig. \ref{fig:identifier_ablation} (b) show that the third identifier $d_g + d_w < \eta$ works best as their overall retraining accuracy is the best across different pruning ratios.

% \vspace{0.2em}
% \textbf{Our GEBT is found to scale up to deep GCNs, of which the experiments are provided in the Appendix}.
